The nEXO Radioassay Program

Material radioactivity compilations, such as the one presented here, are important enablers of science. They are useful for the selection of radiopure materials used in the design and construction of low-energy rare-event search experiments. They allow researchers developing such experiments to save time on material studies and avoid costly duplication of effort. The data presented here were generated in support of the planned nEXO double-beta decay search. This work contains among the most restrictive constraints on the natural radioactivity content of materials of general interest to the low-radioactivity community, found in any tabulation of this kind. In this study, various techniques were employed; they are described here.

==> pgf.tex <==

%\begingroup%
\makeatletter%
%
%
%
%
%
% Filled symbols
%
\DeclareRobustCommand{\tabblackdiamond}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
      \pgfqpoint{-0.035355in}{-0.058926in}%
      }{%
      \pgfqpoint{0.035355in}{0.058926in}%
      }{%
      \pgfpathmoveto{\pgfqpoint{-0.000000in}{-0.058926in}}%
      \pgfpathlineto{\pgfqpoint{0.035355in}{0.000000in}}%
      \pgfpathlineto{\pgfqpoint{0.000000in}{0.058926in}}%
      \pgfpathlineto{\pgfqpoint{-0.035355in}{0.000000in}}%
      \pgfpathlineto{\pgfqpoint{-0.000000in}{-0.058926in}}%
      \pgfpathclose%
      \pgfusepath{stroke,fill}%
      }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
\DeclareRobustCommand{\tabblacksquare}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
      \pgfqpoint{-0.041667in}{-0.041667in}%
      }{%
      \pgfqpoint{0.041667in}{0.041667in}
      }{%
      \pgfpathmoveto{\pgfqpoint{-0.041667in}{-0.041667in}}%
      \pgfpathlineto{\pgfqpoint{0.041667in}{-0.041667in}}%
      \pgfpathlineto{\pgfqpoint{0.041667in}{0.041667in}}%
      \pgfpathlineto{\pgfqpoint{-0.041667in}{0.041667in}}%
      \pgfpathlineto{\pgfqpoint{-0.041667in}{-0.041667in}}%
      \pgfpathclose%
      \pgfusepath{stroke,fill}%
      }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
\DeclareRobustCommand{\tabblackcircle}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
      \pgfqpoint{-0.041667in}{-0.041667in}%
      }{%
      \pgfqpoint{0.041667in}{0.041667in}%
      }{%
      \pgfpathmoveto{\pgfqpoint{0.000000in}{-0.041667in}}%
      \pgfpathcurveto{\pgfqpoint{0.011050in}{-0.041667in}}{\pgfqpoint{0.021649in}{-0.037276in}}{\pgfqpoint{0.029463in}{-0.029463in}}%
      \pgfpathcurveto{\pgfqpoint{0.037276in}{-0.021649in}}{\pgfqpoint{0.041667in}{-0.011050in}}{\pgfqpoint{0.041667in}{0.000000in}}%
      \pgfpathcurveto{\pgfqpoint{0.041667in}{0.011050in}}{\pgfqpoint{0.037276in}{0.021649in}}{\pgfqpoint{0.029463in}{0.029463in}}%
      \pgfpathcurveto{\pgfqpoint{0.021649in}{0.037276in}}{\pgfqpoint{0.011050in}{0.041667in}}{\pgfqpoint{0.000000in}{0.041667in}}%
      \pgfpathcurveto{\pgfqpoint{-0.011050in}{0.041667in}}{\pgfqpoint{-0.021649in}{0.037276in}}{\pgfqpoint{-0.029463in}{0.029463in}}%
      \pgfpathcurveto{\pgfqpoint{-0.037276in}{0.021649in}}{\pgfqpoint{-0.041667in}{0.011050in}}{\pgfqpoint{-0.041667in}{0.000000in}}%
      \pgfpathcurveto{\pgfqpoint{-0.041667in}{-0.011050in}}{\pgfqpoint{-0.037276in}{-0.021649in}}{\pgfqpoint{-0.029463in}{-0.029463in}}%
      \pgfpathcurveto{\pgfqpoint{-0.021649in}{-0.037276in}}{\pgfqpoint{-0.011050in}{-0.041667in}}{\pgfqpoint{0.000000in}{-0.041667in}}%
      \pgfpathlineto{\pgfqpoint{0.000000in}{-0.041667in}}%
      \pgfpathclose%
      \pgfusepath{stroke,fill}%
      }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
%
\DeclareRobustCommand{\tabblackDiamond}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
    \pgfqpoint{-0.058926in}{-0.058926in}%
    }{%
    \pgfqpoint{0.058926in}{0.058926in}%
    }{%
    \pgfpathmoveto{\pgfqpoint{-0.000000in}{-0.058926in}}%
    \pgfpathlineto{\pgfqpoint{0.058926in}{0.000000in}}%
    \pgfpathlineto{\pgfqpoint{0.000000in}{0.058926in}}%
    \pgfpathlineto{\pgfqpoint{-0.058926in}{0.000000in}}%
    \pgfpathlineto{\pgfqpoint{-0.000000in}{-0.058926in}}%
    \pgfpathclose%
    \pgfusepath{stroke,fill}%
    }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
%
\DeclareRobustCommand{\tabblacktriangleright}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
    \pgfqpoint{-0.041667in}{-0.041667in}
    }{%
    \pgfqpoint{0.041667in}{0.041667in}%
    }{%
    \pgfpathmoveto{\pgfqpoint{0.041667in}{-0.000000in}}%
    \pgfpathlineto{\pgfqpoint{-0.041667in}{0.041667in}}%
    \pgfpathlineto{\pgfqpoint{-0.041667in}{-0.041667in}}%
    \pgfpathlineto{\pgfqpoint{0.041667in}{-0.000000in}}%
    \pgfpathclose%
    \pgfusepath{stroke,fill}%
    }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
%
%
%
%
% Open markers
%
\DeclareRobustCommand{\tabdiamond}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
      \pgfqpoint{-0.035355in}{-0.058926in}%
      }{%
      \pgfqpoint{0.035355in}{0.058926in}%
      }{%
      \pgfpathmoveto{\pgfqpoint{-0.000000in}{-0.058926in}}%
      \pgfpathlineto{\pgfqpoint{0.035355in}{0.000000in}}%
      \pgfpathlineto{\pgfqpoint{0.000000in}{0.058926in}}%
      \pgfpathlineto{\pgfqpoint{-0.035355in}{0.000000in}}%
      \pgfpathlineto{\pgfqpoint{-0.000000in}{-0.058926in}}%
      \pgfpathclose%
      \pgfusepath{stroke}%
      }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
\DeclareRobustCommand{\tabsquare}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
      \pgfqpoint{-0.041667in}{-0.041667in}%
      }{%
      \pgfqpoint{0.041667in}{0.041667in}
      }{%
      \pgfpathmoveto{\pgfqpoint{-0.041667in}{-0.041667in}}%
      \pgfpathlineto{\pgfqpoint{0.041667in}{-0.041667in}}%
      \pgfpathlineto{\pgfqpoint{0.041667in}{0.041667in}}%
      \pgfpathlineto{\pgfqpoint{-0.041667in}{0.041667in}}%
      \pgfpathlineto{\pgfqpoint{-0.041667in}{-0.041667in}}%
      \pgfpathclose%
      \pgfusepath{stroke}%
      }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
\DeclareRobustCommand{\tabcircle}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
      \pgfqpoint{-0.041667in}{-0.041667in}%
      }{%
      \pgfqpoint{0.041667in}{0.041667in}%
      }{%
      \pgfpathmoveto{\pgfqpoint{0.000000in}{-0.041667in}}%
      \pgfpathcurveto{\pgfqpoint{0.011050in}{-0.041667in}}{\pgfqpoint{0.021649in}{-0.037276in}}{\pgfqpoint{0.029463in}{-0.029463in}}%
      \pgfpathcurveto{\pgfqpoint{0.037276in}{-0.021649in}}{\pgfqpoint{0.041667in}{-0.011050in}}{\pgfqpoint{0.041667in}{0.000000in}}%
      \pgfpathcurveto{\pgfqpoint{0.041667in}{0.011050in}}{\pgfqpoint{0.037276in}{0.021649in}}{\pgfqpoint{0.029463in}{0.029463in}}%
      \pgfpathcurveto{\pgfqpoint{0.021649in}{0.037276in}}{\pgfqpoint{0.011050in}{0.041667in}}{\pgfqpoint{0.000000in}{0.041667in}}%
      \pgfpathcurveto{\pgfqpoint{-0.011050in}{0.041667in}}{\pgfqpoint{-0.021649in}{0.037276in}}{\pgfqpoint{-0.029463in}{0.029463in}}%
      \pgfpathcurveto{\pgfqpoint{-0.037276in}{0.021649in}}{\pgfqpoint{-0.041667in}{0.011050in}}{\pgfqpoint{-0.041667in}{0.000000in}}%
      \pgfpathcurveto{\pgfqpoint{-0.041667in}{-0.011050in}}{\pgfqpoint{-0.037276in}{-0.021649in}}{\pgfqpoint{-0.029463in}{-0.029463in}}%
      \pgfpathcurveto{\pgfqpoint{-0.021649in}{-0.037276in}}{\pgfqpoint{-0.011050in}{-0.041667in}}{\pgfqpoint{0.000000in}{-0.041667in}}%
      \pgfpathlineto{\pgfqpoint{0.000000in}{-0.041667in}}%
      \pgfpathclose%
      \pgfusepath{stroke}%
      }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
%
\DeclareRobustCommand{\tabDiamond}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
    \pgfqpoint{-0.058926in}{-0.058926in}%
    }{%
    \pgfqpoint{0.058926in}{0.058926in}%
    }{%
    \pgfpathmoveto{\pgfqpoint{-0.000000in}{-0.058926in}}%
    \pgfpathlineto{\pgfqpoint{0.058926in}{0.000000in}}%
    \pgfpathlineto{\pgfqpoint{0.000000in}{0.058926in}}%
    \pgfpathlineto{\pgfqpoint{-0.058926in}{0.000000in}}%
    \pgfpathlineto{\pgfqpoint{-0.000000in}{-0.058926in}}%
    \pgfpathclose%
    \pgfusepath{stroke}%
    }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
%
%
%
%
\DeclareRobustCommand{\tabtriangleright}[1][1.0]{%
\scalebox{#1}{%
  \begin{pgfpicture}%
    \pgfsys@defobject{currentmarker}{%
    \pgfqpoint{-0.041667in}{-0.041667in}
    }{%
    \pgfqpoint{0.041667in}{0.041667in}%
    }{%
    \pgfpathmoveto{\pgfqpoint{0.041667in}{-0.000000in}}%
    \pgfpathlineto{\pgfqpoint{-0.041667in}{0.041667in}}%
    \pgfpathlineto{\pgfqpoint{-0.041667in}{-0.041667in}}%
    \pgfpathlineto{\pgfqpoint{0.041667in}{-0.000000in}}%
    \pgfpathclose%
    \pgfusepath{stroke}%
    }%
    \begin{pgfscope}%
      \pgfsys@transformshift{0in}{0in}%
      \pgfsys@useobject{currentmarker}{}%
    \end{pgfscope}%
  \end{pgfpicture}%
}}%
%
\makeatother%
%
%\endgroup%

